CinePile: A Long Video Question Answering Dataset and Benchmark

Current datasets for long-form video understanding often fall short of providing genuine long-form comprehension challenges, as many tasks derived from these datasets can be successfully tackled by analyzing just one or a few random frames from a video. To address this issue, we present a novel dataset and benchmark, CinePile, specifically designed for authentic long-form video understanding. This paper details our innovative approach for creating a question-answer dataset, utilizing advanced LLMs with human-in-the-loop and building upon human-generated raw data. Our comprehensive dataset comprises 305,000 multiple-choice questions (MCQs), covering various visual and multimodal aspects, including temporal comprehension, understanding human-object interactions, and reasoning about events or actions within a scene. Additionally, we fine-tuned open-source Video-LLMs on the training split and evaluated both open-source and proprietary video-centric LLMs on the test split of our dataset. The findings indicate that although current models underperform compared to humans, fine-tuning these models can lead to significant improvements in their performance.

==> sections/6_discussion_and_conclusion.tex <==
\section{Discussion and Conclusion}
\label{diss_conc}
\vspace{-0.7em}
In this paper, we introduced \logan, a unique long video understanding dataset and benchmark, featuring $\sim$~300k questions in the training set and $\sim$~5000 in the test split. We detailed a novel method for curating and filtering this dataset, which is both scalable and cost-effective. Additionally, we benchmarked various recent commercial video-centric LLMs and conducted a human study to gauge the achievable performance on this dataset. To our knowledge, \logan is the only large-scale dataset that focuses on multi-modal understanding, as opposed to the purely visual reasoning addressed in previous datasets. Our fine-tuning experiments demonstrate the quality of our training split. Additionally, we plan to set up a leaderboard for the test set, providing a platform for new video LLMs to assess and benchmark their performance on \logan. 

Despite its strengths, there are still a few areas for improvement in our dataset, such as the incorporation of character grounding in time. While we believe our dataset's quality is comparable to or even better than that of a Mechanical Turk annotator, we acknowledge that a motivated human, given sufficient time, can create more challenging questions than those currently generated by an LLM. Our goal is to narrow this gap in future iterations of \logan.

\newpage
\section*{Reproducibility Statement}
To ensure the reproducibility of our work, we have taken several steps to provide all necessary details and materials. Our key contributions include: (a) a robust synthetic data generation pipeline for constructing a video question-answering dataset, (b) the final training and test splits derived from this pipeline, and (c) the fine-tuning and evaluation of video language models (LLMs) on these splits. To facilitate replication, we have included the exact prompt used for question-answer generation, the constructed train and test splits, and the fine-tuning and evaluation code in the supplementary materials and appendix.
Specifically, the prompt can be found in Appendix \ref{appendix_sec:qa_prompt}, while the train and test splits are available as Hugging Face objects (\texttt{dataset/cinepile/train} and \texttt{dataset/cinepile/test}) in the provided zip folder. The fine-tuning and evaluation code is also included in the zip folder under the \texttt{code/} directory. We believe these materials, along with the detailed explanations in the appendix and supplementary files, offer a comprehensive source for reproducing our dataset and experiments.

\section*{Ethics Statement}
In accordance with the ICLR Code of Ethics, we acknowledge the potential for biases inherent in large language models, particularly regarding gender, race, and other demographic factors. Given our use of such models to generate question-answer pairs, there is a risk that these biases may be reflected in the generated content, potentially impacting downstream models trained on this data. While we manually reviewed and filtered problematic questions in the evaluation set, the scale of the training set made it infeasible to apply the same level of scrutiny. Additionally, as most of our movie clips originate from the "global west," there is a possibility that certain stereotypes may be perpetuated.
Regarding our human study, we obtained an exemption from our Institute's Review Board (IRB) for the involvement of graduate students. For the dataset release, similar to many existing works \citep{lei2018tvqa,tapaswi2016movieqa,wang2024lvbench,fu2024video}, we plan to release the dataset under the CC-BY-NC-4.0 license, limiting its use to non-commercial, academic purposes. We will host the dataset on Hugging Face, requiring users to agree to the license terms before access. Additionally, We do not distribute any raw video content directly; rather, we provide URLs redirecting to YouTube, ensuring compliance with  YouTube's Terms of Service \citep{youtube_terms}.
